Does My Dog ''Speak'' Like Me? The Acoustic Correlation between Pet Dogs and Their Human Owners

How hosts language influence their pets' vocalization is an interesting yet underexplored problem. This paper presents a preliminary investigation into the possible correlation between domestic dog vocal expressions and their human host's language environment. We first present a new dataset of Shiba Inu dog vocals from YouTube, which provides 7500 clean sound clips, including their contextual information of these vocals and their owner's speech clips with a carefully-designed data processing pipeline. The contextual information includes the scene category in which the vocal was recorded, the dog's location and activity. With a classification task and prominent factor analysis, we discover significant acoustic differences in the dog vocals from the two language environments. We further identify some acoustic features from dog vocalizations that are potentially correlated to their host language patterns.

==> limitations.tex <==
\section* {Limitations}
\paragraph{Dataset Limitation}
We construct the dataset on our own with crawler tool and sound event detection tool. There is noise for two aspects: the first is the video source noise, there are few videos which are not satisfied with our conditions. For example, there are other species of dogs or dogs from unreal environments. The second is that we need a larger dataset, which contains more scenes and clips.


% limitation: dataset noise and size
\paragraph{Analysis Between Dogs and Humans}
For understanding the relationship between voice of dogs and humans at a deeper level, we have analyzed the prominent factors and find the same characteristics between dogs and humans. However, the qualitative analysis is not that descriptive compared to quantitative analysis, which is our future work.

% lack of more straight quantitative analysis between human and dogs

